Weyl singularities in polaritonic multi-terminal Josephson junctions

We study theoretically analog multi-terminal Josephson junctions formed by gapped superfluids created upon resonant pumping of cavity exciton-polaritons. We study the $p$-like bands of a 5-terminal junction in the 4D parameter space created by the superfluid phases acting as quasi-momenta. We find 4/6 Weyl points in 3D subspaces with preserved/broken time-reversal symmetry. We link the real space topology (vortices) to the parameter space one (Weyl points). We derive an effective Hamiltonian encoding the creation, motion, and annihilation of Weyl nodes in 4D. Our work paves the way to the study of exotic topological phases in a platform allowing direct measurement of eigenstates and band topology.

==> unused.tex <==
%We study theoretically cavity exciton-polaritons where gapped superfluids regions of tunable phases are achieved by resonant pumping. This creates analog Josephson junctions where terminal phases act as quasi-momentums so that Andreev bound states analogs form synthetic bands of arbitrary dimension. We study the $p$-like bands of a pentagonal 5-terminal junction (4D space). We show that 3D sub-bands contain either 4 or 6 Weyl points depending if time reversal symmetry is preserved or broken. We connect the topology of real space eigenstates (vortices) to the one of parameter space (Weyl points). We further derive an effective Hamiltonian  describing in the 4D space creation, motion, and annihilation of the Weyl points. This opens perspectives to study exotic topological phases in a platform allowing direct measurement of eigenstates and band topology.

% and might lead to new developments in quantum simulations.

%We show that these bands can cross at WPs. Fixing one phase allows to study 2D bands, which demonstrate non-zero Chern numbers away from Weyl singularities. Two pairs of WPs allow observing $\mathcal{C}=\pm 1,0$. The system is modelled by an effective Hamiltonian based on microscopic considerations. 

%, whereas $\mathscr{N}>2$ can only be solved numerically.

%Moreover, we can vary $\phi_5$ by drawing a horizontal line in Fig.~\ref{fig4}(a), and notice that we can have either 4 or 6 WPs. 6 WPs are impossible if TR symmetry is preserved, which is not the case in general in a 3D subspace of the 4D parameter space. 

%Fig.~\ref{fig4}(a) can be mapped into Fig.~\ref{fig4}(b) when drawing successive horizontal lines. We first cross only four WPs because the change number varies in total by 4. Then, it varies by 6, thus there are 6 WPs.

%This work  paves the way to further studies of WPs and synthetic topological matter using exciton-polaritons, eventually in more than 3 dimensions.

%which strongly restricts the possibilities offered by the topology. An exciting alternative consists in working with synthetic dimensions formed by external parameters that can be tuned at will by experimental conditions.


%Topology is now at the forefront of modern physics. 
%The first topological band gaps were found in the Su-Schrieffer-Heeger unidimensional (1D) chain~\cite{Su1979}. These band gaps are characterized by the Zak phase~\cite{Zak1989} difference, a topological invariant~\cite{Delplace2011}. From then, many systems became known to be topological, and topology as well as topological invariants, such as the Chern number in 2D, became widespread in physics. 
% More generally the key property of topological systems is the existence of topologically protected states robust against some classes of perturbation. 

%described by an effective Hamiltonian arising from the phase dependence of the Andreev reflection. 2D band cuts exhibit Chern numbers $\mathcal{C}=\pm 1,0$ depending on their position with respect to the Weyl points.


% \textit{Origin of the simplified Hamiltonian. --} 
% The simplified Hamiltonian.~\eqref{Ham3D} emulates the situation of the Weyl points at $\phi_2=\pi/2$ and close to this limit in parameter space. First, we will explain the origin of the $\sigma_{x,y}$ terms (which correspond to the in-plane pseudo-spin $(S_1,S_2)$). At $\phi_2=\pi/2$, the $\Tilde{p}$ states are well-defined as $\Tilde{p}_{x,y}$ along the diagonal direction in the $\left (\phi_4,\phi_5\right)$ subspace. For $\left (\phi_4,\phi_5\right)=(0,0)$, the $\Tilde{p}_x$ state is at lower energy whereas at $\left (\phi_4,\phi_5\right)=(\pi/2,\pi/2)$ is is the $\Tilde{p}_y$ state~\cite{suppl}. This implies the bands  must cross twice, which correspond to the Weyl points. From that we can deduce that the $\Delta$ term is due to the control phase $\phi_2=-\phi_3=\pi/2$, and the $\beta(k_x^2+k_y^2)$ term is due to $\phi_4$ and $\phi_5$.  The $\sigma_y$ term can be deduced in a similar way~\cite{suppl}.

%We strongly believe that our system forms an outstanding playground because of the coexistence of Hermitian and non-Hermitian singularities, as well as its experimental accessibility because of the realistic implementation we propose and synthetic topology which is experimentally tunable at will.

%Topological physics relies on the behaviour of the eigenstates of Hamiltonians in a given parameter space, often the reciprocal space. Among the numerous fields of physics where topology is present are superfluid excitations~\cite{Onsager1949,dalfovo1999theory,Pitaevskii}, Landau levels~\cite{thouless1982quantized} and also electronic Bloch bands in solids~\cite{haldane1988model}. \textcolor{red}{Insist on topological bands in reciprocal space and topological invariants}

%Riwar~\textit{et al.} [\textit{Nat. Commun.} \textbf{7}, 11167 (2016)] proposed theoretically a multi-terminal Josephson junction demonstrating synthetic topology in arbitrary dimension, despite the topologically trivial links. We develop an analog of  such junctions in a exciton-polariton system. We find topological bands with non-zero Chern numbers and observe band inversion by the formation of Weyl points. This work deepens the understanding of the topology in multi-terminal Josephson junctions which can be used for 


We find and explain the presence of Weyl points which allow to probe different topological transitions.
%We use realistic parameters to facilitate further experimental implementation.  

% We choose by convention $|u|>|v|$ in the normal region so that $u$ is the majority component and $v$ the minority component. $u(\mathbf{r}),~v(\mathbf{r})$ are propagative states in the normal regions and evanescent in the superfluid gaps. As sketch on Fig. 1(c), a wave of amplitude $u$ and frequency $\omega$ in the normal region reflects on the superfluid gap both at the same frequency (regular reflection) but also toward its time reversal partner at the frequency $-\omega$ and with an amplitude $v$ (Andreev like reflection). In ~\cite{septembre2021parametric}, we considered a 1D system (both in real and synthetic space) which corresponds to the normal incidence case. We found that the regular reflection coefficient does not depend on the superfluid phase whereas the Andreev reflection coefficient contains a factor $e^{\pm 2i\phi}$.


%We now have a 2D real space which requires 
%, as shown in Fig.~\ref{fig1}(a). 
% Qualitatively, the majority component of a bound state of the normal region is close to the one existing in a regular potential well. It is weakly affected by the superfluid phases through the feedback action of the minority component. On the other, the minority Andreev counterpart changes dramatically when tuning the phase difference $\phi$: it is changing symmetry going from a $s$-like shape for $\phi=0$ to a $p$-like shape for $\phi=\pm\pi/2$ which can be quantified for a non-zero Zak phase for the synthetic band.  In this 1D case a topological transition occurs when energy gap between synthetic band closes. Because bare 1D quantum wells states are non-degenerate and well separated in energy, this gap closing only occurs a majority component band cross a minority component band. In fact instead of a crossing, the non-linear non-hermitian coupling between normal and Andreev components makes emerge a pair of exceptional points connected by a Fermi arc \cite{}.





%There are 5 phases among which only three are independent. Thus, the parameter space is of dimension 3 which allows to plot 2D synthetic bands by setting $\phi_2=-\phi_3$ to a given value. It allows to calculate the Berry curvature distribution of the band and finally its Chern number, ultimately determining the topological nature of each band provided it does not cross any other. Following this objective, we will disregard the $\Tilde{s}$ band and its Andreev counterpart because despite they show non-trivial geometry, their topology is trivial (\textcolor{yellow}{see Supplementary materials}). We rather focus on the two $\Tilde{p}$ bands in the $\left (\phi_4,\phi_5 \right )$ subspace ($\phi_2=-\phi_3$ is taken as a parameter). They are plotted in Fig.~\ref{fig2}(a-d) for the same trap size but different $\phi_2$. 





% Fig\ref{fig2}(b) shows the pseudo-spin texture of the lower band. Around the two energy crossing points marked by crossed, it shows a clear winding of the in-plane pseudo-spin. Going slightly apart from $\phi_2=\pi/2$ opens a gap (Fig 2 (c-f)). The band extrema show a non-zero value of the third pseudo-spin component $S_3$ (as also shown on Fig. ?), values which invert passing from slightly below to slightly above $\phi_2=\pi/2$. Fig 2-f shows the pseudo-spin texture on a sphere surrounding the Weyl point in parameter space which demonstrate the typical hedgehog texture.  
% Beyond the two Weyl points crossing at $\phi_2=\pi/2$, the band structure contains two more singularities

 
% The topology of the bands and the induced band gaps is asserted using the Chern number~\cite{berry1984quantal,RevModPhys.82.3045,riwar2016multi}:

% where $S_\phi=[-\pi/2,\pi/2]^2$ is the first synthetic Brillouin zone, and $\mathscr{B}$ the Berry curvature. The latter is computed using the numerical method described in Ref.~\cite{fukui2005chern} (see~\cite{suppl}).
% It is relevant to compute the Berry curvature distribution of isolated bands only when they do not cross. %It is thus possible for $\phi_2 \in ]-\pi/2;\pi/2[ \backslash {0}$. 
% Fig.~\ref{fig2}(e,f) shows the distribution of the Berry curvature of the upper (e) (resp. lower (f)) $\Tilde{p}$ band for $\phi_2=-\pi/3$ and its associated Chern number -1 (resp. +1), which gives a gap Chern number of +1 (the Chern number of the lower band~\cite{suppl}. The distribution of the Berry curvature in the two bands are approximately complementary, the regions where it is concentrated are the same as well as its intensity, but its sign is opposite. In the configuration $\phi_2=\pi/3$, the Chern number associated with the upper (resp. lower) band is +1 (resp. -1), which gives a gap Chern number of -1. Thus, the topology of the gap is different for $\phi_2 \in ]-\pi/2;0[$ and $\phi_2 \in ]0;\pi/2[$. This asserts the existence of topological singularities for $\phi_2=\pm\pi/2$ and $\phi_2=0$ because this is a topological transition across which the gap is forced to close. The evolution of the Chern number of the gap between the two bands with respect to $\phi_2$ is shown in Fig.~\ref{fig2}(g): There are two regions of different topology, and going from one to the other is possible only by passing through a topological singularity.


% We remind that a wave of positive energy $+E$ going from a normal to a superfluid region is reflected both at $+E$ with wavevector (specular reflection) and at $-E$ (Andreev reflection). This is modeled by the scattering formalism, involving reflection coefficients quantifying the proportions of each reflection process~\cite{septembre2021parametric}:
% \begin{equation}\label{refl-coeffs}
%   \begin{array}{r c l}
%       r_N & = & \frac{(k_I-i\kappa_-)(k_A+i\kappa_+)|u|^2 + (k_A+i\kappa_-)(k_I-i\kappa_+)|v|^2}{ (k_I+i\kappa_-)(k_A+i\kappa_+)|u|^2 + (k_A+i\kappa_-)(k_I+i\kappa_+)|v|^2},\\
%     r_A & = & \frac{2 i \sqrt{k_I k_A} (\kappa_+-\kappa_-) |u||v| }{ (k_I+i\kappa_-)(k_A+i\kappa_+)|u|^2 + (k_A+i\kappa_-)(k_I+i\kappa_+)|v|^2}e^{-2i\phi}.
%   \end{array}
% \end{equation}

% We first consider Andreev reflection in 2D under arbitrary incidence angle. For an incoming particle of positive energy of wavevector  $\mathbf{k}_I \cdot \mathbf{x}=k_I$, a particle is reflected at the opposite energy at wavevector $\mathbf{k}_A \cdot \mathbf{x}=k_A$ because of Andreev reflection. The specular and Andreev reflection coefficients can be found from the continuity of the wave function and its derivative at the interface~\cite{septembre2021parametric}:
% \begin{equation}\label{refl-coeffs}
%   \begin{array}{r c l}
%       r_N & = & \frac{(k_I-i\kappa_-)(k_A+i\kappa_+)|u|^2 + (k_A+i\kappa_-)(k_I-i\kappa_+)|v|^2}{ (k_I+i\kappa_-)(k_A+i\kappa_+)|u|^2 + (k_A+i\kappa_-)(k_I+i\kappa_+)|v|^2},\\
%     r_A & = & \frac{2 i \sqrt{k_I k_A} (\kappa_+-\kappa_-) |u||v| }{ (k_I+i\kappa_-)(k_A+i\kappa_+)|u|^2 + (k_A+i\kappa_-)(k_I+i\kappa_+)|v|^2}e^{-2i\phi}.
%   \end{array}
% \end{equation}
% The key feature is the appearance of the phase $\pm 2i\phi$ in the Andreev reflection coefficient $r_A$, as in the 1D case.
% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=0.99\linewidth]{fig3.pdf}
%     \caption{The interplay of the $p_x$ and $p_y$ orbitals and the phases of the reflection coefficients in the synthetic space formed by $\phi_4$, $\phi_5$ (arrows). (a,b) The $p_x$ orbital; (c,d) the $p_y$ orbital, plotted for the Brillouin zone center (a,c) and corner (b,d). Opposite orientation of the phases increases the mode energy in (b) and (c). }
%     \label{fig5}
% \end{figure}

% We start with the in-plane pseudo-spin of~\eqref{Ham3D} described by the matrices $\sigma_x$, $\sigma_y$ and corresponding to the $p_x$, $p_y$ orbitals and their diagonal superpositions $p_x \pm p_y$. Figure~\ref{fig3} shows the calculated images of the $p_x$ and $p_y$ orbitals ($|\psi(x,y)|^2$ represented by false color) together with the five phases of the Andreev reflection coefficients (double of the respective phases) represented by arrows. The relative phase at the faces in the main orbital direction (red arrows) controls the energy of the state. In panels (a) and (d) all red arrows point in the same direction (zero phase difference): it is therefore the state $p_x$ which has the lowest energy at the center of the Brillouin zone and the state $p_y$ at its corner. In  panels (b) and (d) the orientation of the red arrows is opposite, corresponding to the maximal relative phase and maximal energy. The respective symmetry of the orbitals and the faces are therefore at the origin of the $\sigma_x$ term in \eqref{Ham3D}: the $\Delta$ term is due to the control phase $\phi_2=-\phi_3=-\pi/2$ (panels a,c), and the $\beta(k_x^2+k_y^2)$ term is due to $\phi_4,\phi_5$ (panels a,b). Since the splitting between the $p_x$ and $p_y$ modes changes sign between the center and the corner of the Brillouin zone, it must cross zero: this is the Weyl point. The $\sigma_y$ term can be deduced in a similar way~\cite{suppl}.


























% A 1D junction such as the one described in~\cite{septembre2021parametric} and depicted in Fig.~\ref{fig1}(a) essentially forms a quantum well. The mode of lowest energy is a $s$-like state (denoted $\Tilde{s}_{1D}$) as shown in blue in Fig.~\ref{fig1}(b,c). Because of the Andreev reflection process occurring at the interfaces between normal and superfluid regions, there exist a Andreev counterpart of this $\Tilde{s}_{1D}$ state which is also confined in the junction: The states always come in pairs: The first one is the state coming from the quantum confinement (induced by the interactions, see Eq.~\eqref{BdG0}), the second one is appearing from the parametric processes linked to successive Andreev-like reflections, as described in Ref.~\cite{septembre2021parametric}. When tuning the phase difference between the two superfluids that form the junction, the quantum confined state and its Andreev counterpart act differently. The shape of the first one is not affected too much by a non-zero phase, as shown in Fig.~\ref{fig1}(b,c) because it only gives an additional phase to the wave function. The shape of the mode remains $s$-like, but it acquires a phase $e^{2i\phi}$, where $\phi$ denotes the phase difference between the two superfluids. However, its Andreev counterpart changes dramatically when tuning the phase difference $\phi$: it goes from a $s$-like shape for $\phi=0$ to a $p$-like shape for $\phi=\pm\pi/2$. 
%Solving numerically the Eq.~\eqref{BdG0} gives the energy of bound states $E=\hbar\omega$ with respect to the laser detuning $E_p=\hbar\omega_p$ and phase difference $\phi$. It allows to plot the energy of a bound state with respect to the phase difference (which forms synthetic bands), where the changes of shape of the Andreev counterpart of each band translate into a non-zero Zak phase in the 1D junction as shown in Ref.~\cite{septembre2021parametric}. 



 %A 1D junction such as the one described in~\cite{septembre2021parametric} and depicted in Fig.~\ref{fig1}(a) essentially forms a quantum well. The mode of lowest energy is a $s$-like state (denoted $\Tilde{s}_{1D}$) as shown in blue in Fig.~\ref{fig1}(b,c). Because of the Andreev reflection process occurring at the interfaces between normal and superfluid regions, there exist a Andreev counterpart of this $\Tilde{s}_{1D}$ state which is also confined in the junction. 
%Each mode is composed by a majority component of frequency $\omega$ and amplitude $u$. When this wave is reaching the pumped superfluid area, it undergoes an elastic regular reflection on the superfluid which acts as a potential barrier. It also undergo a non-linear coupling toward its time reversal partner at frequency $-\omega$ and with an amplitude $v$ ($|v|<|u|$). 

 %The superfluid phases therefore appear as external gauge fields acting on the bound states located in the normal region. It explains why these bound states can change symmetry along the synthetic bands and be topologically non-trivial.  
 
 
% Now we focus on the two $\Tilde{p}$ bands. In a 2D quantum well with central symmetry, the two $\Tilde{p}$ states should be degenerate regardless of its precise shape. In our case, the two $\Tilde{p}$ states form synthetic bands. We will study the behavior of the crossing points between the two $\Tilde{p}$ bands. We state that the $\Tilde{p}_x$ state only ''sees'' the phase difference along $\textbf{x}$ (denoted $\mathbf{\Phi_x}$) whereas $\Tilde{p}_y$ only feels $\mathbf{\Phi_y}$. The energy of the state depends strongly on the phase (as shown previously, and also analytically in Ref.~\cite{septembre2021parametric}). Thus, for the states to be degenerate, the phase differences along the two directions should be null:
% \begin{equation}
%     \mathbf{\Phi}=\begin{pmatrix}\Phi_x \\ \Phi_y\end{pmatrix}=\textbf{0}.
% \end{equation}
% The vector $\mathbf{\Phi}$ is defined as:
% \begin{equation}\label{sum}
%     \mathbf{\Phi}=\sum_{i=1}^\mathscr{N} \phi_i \mathbf{n}_i,
% \end{equation}
% where $\mathbf{n}$ is the vector normal to the interface going toward the normal region. This ultimately gives:
% \begin{equation}\label{eqphi}
%     \begin{array}{rcl}
%          \phi_4 & = & \phi_2+\varphi\phi_3  \\
%          \phi_5 & = & \phi_3+\varphi\phi_2
%     \end{array}
% \end{equation}
% where $\varphi$ is the golden ratio, appearing here only because of the pentagonal shape of the normal region. We remind here that the phases $\phi_i$ are defined modulo $\pi$ (see Eq.~\ref{BdG0}), thus the system is more complex than it appears.

% Our superfluids are broad regions of space whereas the superconducting links considered in Ref.~\cite{riwar2016multi} are not. Thus, among the $\mathscr{N}=5$ phases, we have to take two phase references for the two directions $x$ and $y$.  We recall that $\phi_1=0$ for the $x$ direction and $\phi_2=-\phi_3$ which ultimately sets a phase reference in the $y$ direction. \textcolor{green}{Note that this is not a unique way to define phase references~\cite{suppl}}, but this will be the only one considered in this work.
% Thus, the space of independent phases is of dimension $\mathscr{N}-2=3$. Setting $\phi_2$ to a given value allows to plot 2D energy bands, where $\phi_4$ and $\phi_5$ play the roles of parameters.

% The first situation considered is $\phi_2=\phi_3=0$. This leads to the bands plotted in Fig.~\ref{fig2}(a). Eq.~\eqref{eqphi} naturally gives the crossing point at $(\phi_4,\phi_5)=(0,0)$. The numerical experiment follows this with a slight error coming from the square mesh which cannot properly fit the pentagonal shape \textcolor{green}{(see Supplementary)}: there are two crossing points instead of the unique double degeneracy point expected. From this configuration, moving slightly in the parameter space removes instantaneously the degeneracy. We deduce that this degeneracy is a Weyl point indeed. 
% As a second configuration, we consider $\phi_2=-\phi_3=-\pi/2$ which is at the border of the synthetic Brillouin zone. This gives birth to two clearly separate linear crossing points, as shown in Fig.~\ref{fig2}(b). Again, moving slightly in the parameter space removes the degeneracy: Theses points are Weyl points indeed. From equation~\ref{eqphi}, we can calculate the analytical position of the crossing points and find a small deviation that we assume come from the broadening of the superfluid regions which are not perfectly fitted by the model of Eq.~\eqref{sum}.
% Following this study, we can compile the result in Fig.~\ref{fig2}(c) which shows the parameter space for both analytical and numerical results. We can clearly see the Weyl points occuring in the two situations described before. The agreement between numerics and analytics is not perfect.


\emph{Weyl exceptional rings.--}
The Eq.~\eqref{BdG0} contains a non-Hermitian matrix. Usually, Weyl (or Dirac) points are observed only in Hermitian systems~\cite{lu2015experimental,noh2017experimental}, and non-Hermiticity makes them split in two exceptional points~\cite{Voigt1902,PhysRevLett.123.227401,PhysRevLett.123.237202} which eventually annihilate~\cite{krol2021annihilation} or form a ring of exceptional points~\cite{zhen2015spawning} or Weyl exceptional rings~\cite{PhysRevLett.118.045701,cerjan2018effects,cerjan2019experimental} that were found to exist in synthetic dimensions recently~\cite{li2021experimental} depending on the nature of the perturbation~\cite{bergholtz2021exceptional}. In our non-Hermitian system, we have access to both Hermitian singularities (Weyl points) and non-Hermitian singularities: Weyl exceptional rings, which makes it a beautiful and original playground.

In 1D~\cite{septembre2021parametric}, we demonstrated that tuning the size of the trap $a$ allowed the bands to cross and form exceptional points. As explained previously, our junction forms a quantum well that confines states. The energy of the confined states decrease when the trap size increases~\cite{}. On the contrary, the Andreev counterpart of the confined states has opposite energy: Its energy increases when the trap size increases. Thus, a state and its Andreev counterpart become resonant at null energy (corresponding to the pump energy $E_p$). Another situation is the resonance between a state and the Andreev counterpart of another state ($\Tilde{s}$ state and the Andreev counterpart of $\Tilde{p}$ state for instance) which occurs at not-null energies. Both types of resonances lead to the formation of exceptional points and parametric amplification.

With 3 parameters instead of 1, the exceptional points turn out to be the 1D projections of a Weyl exceptional ring. Fig.~\ref{fig3} shows the real part (a) and imaginary par (b) of the energy for the two bands that merge, here the lowest $\Tilde{p}$ and the Andreev counterpart of the $\Tilde{s}$ band (the two $\Tilde{p}$ bands are not degenerate because we set on purpose $\phi_2=-\pi/3$). The bands merging is the non-Hermitian equivalent of crossing~\cite{bergholtz2021exceptional} and the specific behaviour of our bands is shown in \textcolor{green}{supplementary}. The two bands are degenerate in a wide region, where their imaginary parts are different (opposite in our model, see Eq.~\eqref{GP}). This leads to amplification~\cite{septembre2021parametric} of half of the states. On the contrary, there is still a convex region where the real part of the energy is not degenerate. The two regions form an interface which is precisely the Weyl ring of exceptional points. \textcolor{green}{Its precise geometry is described in supplemental materials.} Along this line, both real parts and imaginary parts of the energy are degenerate (more precisely, the eigenstates and eigenvalues coalesce). Thus, this ring is a ring of exceptional points indeed.


\emph{Discussion.--} We want to stress that the Weyl ring we observe here is not the non-Hermitian counterpart of the Weyl points discussed previously. In general, the Weyl points of a Hermitian system can transform in Weyl rings by adding the proper non-Hermitian ingredient~\cite{bergholtz2021exceptional,yan2021unconventional}. This is not what can be done in our system. Our intrinsically non-Hermitian system can host both Hermitian and non-Hermitian singularities by itself. The Hermitian singularity consists in the crossing of two bands of same nature: Either two ''main bands'' coming from quantum confinement in the trap, or two Andreev counterparts. In this case, the Andreev process is involved only to bring the additional phases of the superfluids to the wavefunction, which explains the Hermitian nature of the singularities. On the other hand, the non-Hermitian singularities and band merging arise when a ''main band'' coming from quantum confinement in the trap meets an Andreev counterpart band (either its own one, at zero energy, or the Andreev counterpart of another band, at non-zero energy). In this case, Andreev process is more crucial because it makes appear a second band to each band coming from quantum confinement. In our system, this Andreev process is linked to a non-Hermitian matrix~\eqref{BdG0} which explains the non-Hermitian nature of this singularities.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.9\linewidth]{}
    \caption{(a) Normalized real part of the energy of a $\Tilde{p}$ band and the Andreev counterpart of the $\Tilde{s}$ one during their merging (crossing with non-Hermiticity). (b) Imaginary part of the same bands. The cyan ellipse fits the Weyl ring where both real and imaginary parts of the energy coalesce.}
    \label{fig3}
\end{figure}

%Besides being related to the specific properties of metal superconductors microconstructions \cite{blonder1982transition,pannetier2000andreev}, direct observation of this retro-reflection process has been reported in superconductors \cite{Benistant83} and liquid Helium-$3$\cite{Enrico1993}. 



%Andreev process can also lead to specular reflection when dealing with relativistic electron dispersions as in graphene \cite{beenakker2006specular}. Similarities and differences between BECs and superconductors have already been noticed in the context of coherent Josephson oscillations observed both in cold atoms \cite{Albiez2005} and cavity polaritons systems \cite{Sarchi2008,Shelykh2008,abbarchi2013macroscopic}. Scattering of density waves in BECs has also been widely considered in the context of analog Hawking radiation in 1D sonic black holes \cite{Recati2009,Macher2009}.
%A similar effect, known as optical phase conjugation, has been discovered and studied in the 70's in nonlinear optics  \cite{yariv1978phase}. In this context, an incident optical wave arriving on a phase conjugating mirror (which involves nonlinear processes) is reflected as its time reversed partner, meaning that the reflected wave has the same frequency and opposite wavevector. The analogy between optical phase conjugation achieved using degenerate four wave mixing and the electronic Andreev reflection has been noticed and discussed in refs \cite{van1991andreev,PhysRevA.56.4216}.

%Andreev bound states emerge in SNS junctions, that is, two superconducting media surrounding a normal one \cite{wendin1996giant,chevallier2012mutation,sothmann2016fingerprint}. Similarly to the textbook case of the quantum well, such systems host bound states. However, thanks to the specific properties of the Andreev reflection, some smartly-designed junctions accommodate non-trivial topological Andreev bound states. Topology is a burgeoning topic in physics~\cite{kosterlitz1973ordering, thouless1982quantized,berry1984quantal,haldane1988model} which was first introduced to explain the integer quantum Hall effect, and finally extended to many domains in solid-state physics or in photonics \cite{haldane2008possible, raghu2008analogs}, giving birth to topological insulators \cite{bleu2016interacting,langbehn2017reflection,serra2018observation,mukherjee2020observation} or topological lasers \cite{solnyshkov2016kibble,st2017lasing, bahari2017nonreciprocal,bandres2018topological} for instance, as well as topological Josephson junctions~\cite{oreg2010helical,lutchyn2010majorana,rokhinson2012fractional,mourik2012signatures, nadj2014observation,albrecht2016exponential, bocquillon2017gapless, le2019joule}.

%Nowadays, exciton-polariton systems are widely studied for their possibility to form topological insulators \cite{nalitov2015polariton,bardyn2015topological,karzig2015topological,klembt2018exciton}. Actually, polaritons stand for a very powerful platform in many domains because they allow a large diversity of applications, among which bright solitons \cite{egorov2009bright,sich2012observation}, soliton-based four-wave mixing \cite{yulin2004four,skryabin2005theory,gorbach2006four} or even an optical parametric oscillator (OPO) behaviour \cite{savvidis2000angle,baumberg2000parametric,kavokin2017microcavities}. Furthermore, they can also be used in analogue physics, for instance in analogue gravity \cite{jacquet2020polariton}.

%In this letter, we consider a peculiar configuration of a driven dissipative superfluid, a regime achievable in state-of-the-art exciton-polariton experiments \cite{amo2009superfluidity,hivet2012half,boulier2015vortex}.
%In particular, a driven superfluid can give rise to a gapped spectrum of its excitations analogous to the pairing gap of a fermionic superfluid contrary to the optical phase conjugation where the spectrum in the "mirror" is gapless (which leads to the possibility of amplified transmission which will not be the case here). This is basically an analogue of the Andreev reflection which differs from the one theoretically proposed for a scheme with a decaying atomic condensate in \cite{Zapata2009}, which to our knowledge has never been experimentally observed yet.
%Moreover, inspirited by a recent theoretical proposition \cite{riwar2016multi} on the possibility to probe artificial topological matter using multi-terminal superconductor Josephson junctions, we also study the bosonic analog of Andreev bound states in a Superfluid - Normal - Superfluid (SNS) junction, a problem never considered before to our knowledge. The system is thus similar to the one studied in\cite{goblot2016phase} but with linear states. We finally discuss the possibility to get an OPO on a topologically protected linear state.

Fig.~\ref{fig4} (a) shows a scheme which allows to create an "interface" in the parameter space between regions of opposite topology.  
 
 
 
%Therefore, an interface between two junctions with different gap topologies (for instance one junction with a topologically trivial gap and the other one with a topologically-non trivial gap) must exhibit a point where the gap is zero, which is a topologically-protected interface state. Actually, increasing the normal region width indeed modify the Zak phase of given bands, as shown by Fig.~\ref{fig3}.

 
%In this specific case, an appropriate definition of the wavefunction in the normal region is:
% \begin{equation}\label{psiN}
%     \psi_N=\begin{pmatrix} Ae^{ik_1x} + Be^{-ik_1x}\\ 
%     Ce^{ik_2x} + De^{-ik_2x}\end{pmatrix},
% \end{equation}
% where $A,~B,~C,~D$ are general coefficients.

% In this case, the bands looks similar to the bands of the SSH model. However, their behaviour is largely different. The bands exist for precise domains of width of the normal region. As two bands get closer and touch, they combine and their energy becomes complex in this precise domain.




Finally, these junctions display an optical parametric oscillator (OPO) behaviour. As aforementioned, the topology of the bands dramatically change when the normal region width is modified. It implies that for critical values of $a$, there is a topological transition between states. This is akin to the works of \cite{bernevig2006quantum,konig2007quantum}. This gives birth to exponentially growing modes and therefore an OPO. The Fig.~\ref{fig4} shows that when the energy of two states are the exact complementary of the pump frequency and symmetrical with respect to it, the OPO appears. The linear state is indeed exponentially growing. The energy conservation gives:
\begin{equation}
    2 \omega_p= \left ( \omega_p - \delta \omega \right ) + \left ( \omega_p + \delta \omega \right )
\end{equation}
The energy conversion is thin because  the only appropriate energies to consider are inside the gap, which is of the order of magnitude of the pump energy, that is, typically around hundreds of $\mu$eV.



%Importantly bogolons energies can take complex values. A positive imaginary part will be associated with the development of exponentially growing modes which formally makes the perturbative approach we use not valid anymore.

%Here, the coefficients $u,~v$ are the Bogoliubov coefficients and stand for the quantity of the quasiparticle at each energy ($E,~ -E$ respectively). In other words, there are four Bogoliubov coefficients in the superfluid region $u_\pm,~v_\pm$ that encode the proportion of wavefunction at each energy ($u_\pm$ at $+E$, $v_\pm$ at $-E$) and at each characteristic length ($u_+,~v_+$ at $\kappa_+$, $u_-,~v_-$ at $\kappa_-$).
%Dealing only with positive energies $E>0$, the normalisation condition:
%\begin{equation}
  %  E|u_\pm|^2-E|v_\pm|^2 = \mp E
%\end{equation}
%means that the energy carried by a single bogolon at a frequency $\omega$ is $E=\hbar\omega$. The Bogoliubov coefficients in the evanescent case can finally be computed:


%The Bogoliubov-de Gennes equations usually describe the electron/hole symmetry. In our case, the so-called particles and "holes" share the same nature and are only different in energy (except for $E=0$). Therefore, their group velocity is different in general.


The ratio between them has a theoretical limit of $2$ for tiny $\alpha n$.

%The bosonic analogue of the Andreev reflection that we propose to study occurs in an optical cavity, at the interface between a normal region and a superfluid one. In the normal region, the dispersion is parabolic which is typical for massive quasiparticles while in the superfluid one, a gap separates the two branches. These considerations are schematically plotted in Fig.~\ref{fig1}. In the gap, there is no available propagative states but only evanescent ones. This energy spectrum qualitatively resembles the one of superconductors, the pump energy playing here the role of the Fermi energy in the electronic case.




%Andreev developed a theory on the reflection of an electron in a hole at a superconductor interface~\cite{andreev1964thermal}, which was apparently totally disconnected from topology.

%Important efforts are made to implement them \cite{draelos2019supercurrent,Pankratova2020} because the system is of crucial interest in the field of quantum correlations for instance~\cite{boogers2021holonomic,PhysRevResearch.4.013038}.

%The Andreev physics (Andreev reflection and Andreev bound states) raise a huge interest in fundamental physics in a large variety of research fields, ranging from cosmology to photonics. For instance, Andreev reflection is well-known to be very akin to phenomena encountered near the horizon of black holes~\cite{PhysRevD.53.7082,PhysRevB.100.245436,PhysRevD.96.124011,PhysRevD.102.064028}. Analogue physics allows to investigate the properties of inaccessible systems such as black holes in this case.

%However, one major drawback of investigating electronic states is the impossibility to measure directly their wave-function. Fortunately enough, there exists a photonic analogue of Andreev reflection~\cite{Zapata2009} where the wave-functions themselves are supposed to be experimentally accessible. Moreover, a theoretical analogue of Josephson junctions exists in cavity exciton-polaritons~\cite{septembre2021parametric} in 1D. The experimental implementation can be envisioned in 2D as well because of the experimental possibilities offered by the platform~\cite{goblot2016phase,Koniakhin2019,claude2020taming} under resonant driving~\cite{Carusotto2013,kavokin2017microcavities}, which would allow to study analogs of multi-terminal Josephson junctions.
%By resonantly driving the cavity~\cite{Carusotto2013,kavokin2017microcavities}, a gap opens in the energy spectrum which corresponds to the formation of a ``gapped superfluid'', very akin to the superconducting regime. Modulating  the pump intensity in space is possible, which allows to form two or more gapped regions with controllable phase,  separated by normal non-superfluid regions \cite{goblot2016phase,Koniakhin2019,claude2020taming}, that is, an outstanding analogue of a multi-terminal Josephson junction.

%Typical bands are shown in Fig.~\ref{fig1}(d) in a configuration where the junction hosts only the first band ($\sim s$ band) and its Andreev counterpart. The latter clearly has a non-trivial behavior because the state is absolutely not constant along the band. It varies continuously from an almost pure $p_x$ state on the corners to an approximate $s$ state on the center of the parameter space, while being mixed with a $p_y$ state at the edges. This conclusion is totally in agreement with what was found in 1D~\cite{septembre2021parametric}.


%\emph{Topology.--}
%We consider a square trap formed by 4 links as depicted in Fig.~\ref{fig1} \textcolor{green}{(see Supplemental for a different configuration)}. The space of independent parameters (phases) is thus of dimension 3. We consider a larger trap than previously ($2a=1.6~\,\mu$m) in order to have both $s$ and $p$ bands (and their Andreev counterparts). First, note that the $p$-branches as well as their Andreev counterparts are degenerate in one (or two) point(s) of the parameter space, when the phase difference of the facing edges in the $x$ direction are the same (in absolute value) as the ones in the $y$ direction. This can be easily understood by symmetry considerations. Fig.~\ref{fig2}(a,c-f) show the bands in the parameter space for $\phi_2=\phi_1$ with their associated states. We can see in Fig.~\ref{fig2}(c) that the $p$ bands are mixed, that is, there is no $p_x$ and $p_y$ bands but rather a linear combination of the two states. In Fig.~\ref{fig2}(d), we see that the bands are neither well-defined in terms of vortex/antivortex decomposition. However, in some domains, the states can be described as vortices or antivortices (green/blue in this panel, respectivley). These real-space topological singularities carry a $\pm 1$ (respectively) winding number:

% where $\mathbf{dr}$ forms a close loop around the center of the phase singularity (abrupt change of $2\pi$) in the counter-clockwise direction.
% \textcolor{blue}{Making a 2D cut along $\phi_5=0$ allows to see that there is indeed a $p_x$ band above the $p_y$ band, and \textit{vice versa} for $\phi_3=0$. Indeed, if the facing phases along a given direction are equal, the $p$ state along this direction is lower in energy, and the state is forced by symmetry to be either purely $p_x$ or $p_y$.}
% This is very different from the 1D case~\cite{septembre2021parametric} where there is only one $p$ state. Thus, it is not in contradiction of what has been observed in 1 dimension but rather an extension of it to higher dimensions, where there is one $p$ state for each direction. However, the states corresponding to the Andreev counterpart of the $p$ bands change more dramatically indeed. As shown in Fig.~\ref{fig2}(e,f) with the $p_{x,y}$ or vortex/antivortex basis (respectively), the states have three major components, as the Andreev counterpart of the $s$ band, which are this time $p_{x,y}$ and \textcolor{blue}{$s$ or $d$ for the upper/lower band respectively}.
% \textcolor{blue}{We clearly see that the system hosts real space topological singularities (\emph{vortices}~\cite{}). %that can be created or annihilated by tuning the phases of the pumps. 
% The (anti-)vortices correspond to a quantized orbital angular momentum (OAM)~\cite{} $l=1$ ($l=-1$ for antivortices), which is calculated by:
% \begin{equation}
%     l=\oint\arg \psi (\textbf{r}) \textbf{dr}.
% \end{equation}
% The OAM is associated to the states in the figure. We can see that depending on the phase, there is a possibility to create or annihilate (anti)vortices, which is accompanied by a quantized change of the OAM.}
%\cite{silveirinha2019quantized}
%Thus, the creation and annihilation of vortices is accompanied by a quantized variation in the orbital angular momentum of the state.

% To quantify the change of the states with the phases, we compute the Berry curvature $\mathscr{B}(\phi_\mu,\phi_\nu)$ (where $\mu,~\nu$ are the indices of the varying phases) by the numerical method described in Ref.~\cite{fukui2005chern} \textcolor{green}{(see Supplemental for more details)}. This allows to calculate the Chern number~\cite{berry1984quantal,RevModPhys.82.3045,riwar2016multi}:
% \begin{equation}
%     \mathscr{C}=\frac{1}{2\pi}\iint_{S_\phi} \mathscr{B}(\phi_\mu,\phi_\nu)\, d\phi_\mu\,d\phi_\nu,
% \end{equation}
% where $S_\phi=[-\pi/2,\pi/2]^2$ is the first synthetic Brillouin zone, which ultimately determines the topology of the system. Obviously, there is barely no change in the state for the $s$ band, so the Berry curvature distribution is trivial as well as the Chern number. On the other hand, the $p$ bands and their Andreev counterparts cross, thus making impossible to define the Berry curvature. For the Andreev counterpart of the $s$ band, the computation is feasible and gives the results shown in Fig.~\ref{fig2}(b). The Berry curvature is clearly non-trivial because the state changes, as aforementioned. However, the positive and negative contributions compensate each other and finally give a trivial Chern number $\mathscr{C}=0$. 
% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{fig2v1.pdf}
%     \caption{(a) $s$ band and its Andreev counterpart. (b) Berry curvature distribution of the Andreev counterpart of the $s$ band in the parameter space. (c-f) $p$ bands and their Andreev counterparts. For all panels, the junction has 4 terminals, $\phi_2=\phi_1$, $2a=1.6\,\mu$m. False colors correspond to the decomposition of the state on a given state basis (see colormaps for precisions).}
%     \label{fig2}
% \end{figure}
%We can explore other configurations by tuning the phase $\phi_2$ instead of $\phi_5$. \textcolor{green}{However, they are of equal interest in terms of topology, as briefly discussed in the supplemental.}

%Overall, a 4-terminal junction is always topologically trivial in our case, even if the geometry of eigenstates has a non-trivial behavior. This constrats with the electronic multi-terminal Josephson junctions~\cite{riwar2016multi}. In this article, the authors use a numerical method to create random scattering matrices connecting the links, and few of them ($\sim 5\%$) give birth to zero-energy Weyl points and a non-trivial topology even with 4 links and even with 3 terminals~\cite{Meyer2017,xie2017topological} (both with only one channel).



%Now, we focus on a 5-terminal junction ($\mathscr{N}=4$). In general, most of the features described previously still hold, whereas this configuration also allows to explore a regime where the Chern number is non-zero. We keep three constant phases (still with $\phi_1=0$ as a reference) whereas the two others vary, allowing to plot 2D-bands. Fig.~\ref{fig3}(a) shows the configuration considered: the constant phases are $\phi_{2,3}=\phi_1\pm \pi/4$ creating a robust phase gradient. \textcolor{green}{Other choices of phases are shown in the supplemental}, but they globally correspond to the 4-terminal case, their topology being trivial.

%These values for the constant phases strongly modifies the behavior of the $p$ bands and their Andreev counterparts. 
%The $s$ band is shown by Fig.~\ref{fig3}(b) where the band is plotted with its Andreev counterpart. Note that the bands are inverted with respect to Fig.~\ref{fig2}(a): the $s$ band is at negative energy whereas its Andreev counterpart is at positive ones. Fig.~\ref{fig3}(c) depicts the Berry curvature of the Andreev counterpart of the $s$ band, which is non-trivial but globally symmetric, thus giving a zero Chern number. However, these values of the constant phases strongly modifies the behavior of the $p$ bands and their Andreev counterparts. The original bands are not anymore an arbitrary combination of $p_x$ and $p_y$ states but each band can be associated to a vortex (lower band) or antivortex (upper band) state, respectively, as shown by Fig.~\ref{fig3}(d). The bands are separated because contrary to $p_x$ and $p_y$ states (in the absence of phase gradient), vortices and antivortices are not degenerate. The interaction between the bands when they get closer is strong enough to mix make a vortex state appear in the antivortex band, and \textit{vice versa}. This shows through the Berry curvature distribution (Fig.~\ref{fig3}(e)) which is non-symmetric and strongly localized close to the anticrossing point. Thus, the Chern number of the two bands in non-trivial: $\mathscr{C}=+1$ for the vortex band and $\mathscr{C}=-1$ for the antivortex band. The Andreev counterparts of the bands being the exact symmetric with respect to the pump energy of their corresponding original state, they also show a gap between them (see Fig.~\ref{fig3}(f) where the Andreev bands are plotted). The behavior of the states along the bands is complex, however the Berry curvature distribution clearly shows that it is topologically non-trivial, each band being associated with a non-zero Chern number. The Berry curvature of each band is plotted in Fig.~\ref{fig3}(g)  The Andreev counterpart of the vortex band carries a Chern number $\mathscr{C}=-1$ whereas the one of the antivortex carries a Chern number $\mathscr{C}=+1$, that is, strictly the opposite of their corresponding original band. The topologically non-trivial behavior of our bands is consistent with the topology of the bands in electronic multi-terminal Josephson junctions~\cite{riwar2016multi}. Furthermore, our understanding of the vortices-based topology may even explain how the bands are found topological in this electronic system, where the states are not accessible.
%However, it seems to be more restricted in our polaritonic system because the total Chern number of the bands is zero, even if some gaps have a non-zero Chern number. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ============================ H ============================ %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \emph{Simplified Hamiltonian.--} Considering Fig.~\ref{fig2}(a) together with Fig.~\ref{fig3}(a,b), we note that the whole 3D reciprocal space close to the WP ($\phi_2=\pi/2$) can be described by the following simplified $2\times2$ Hamiltonian. Defining alternative parameter space vectors $k_x \equiv \phi_3 - \phi_4$, $k_y\equiv \phi_3 + \phi_4$ and $k_z\equiv \phi_2-\pi/2$, it reads:
% \begin{eqnarray}
%     \hat{H}&=&-\left[\left(\Delta-\beta\left(k_x^2+k_y^2\right)\right)\sigma_x+2\beta' k_x k_y \sigma_y \right. \nonumber\\
%     &+&\left.\left(\alpha k_x+\xi k_z\right)\sigma_z\right],
%     \label{Ham3D}
% \end{eqnarray}
% where $\sigma_{x,y,z}$ are the Pauli matrices. The microscopic origin of all terms in this Hamiltonian is discussed in~\cite{suppl}. Qualitatively, the $\sigma_x$ and $\sigma_y$ terms are due to the energy change with the phase difference, whereas the $\sigma_z$ terms are due to the Josephson currents.
% The $\Delta$ and  $\beta$ with $\sigma_x$ describe the inversion of the energies of the $\Tilde{p}_x$ and $\Tilde{p}_y$ between the center and the corners of the Brillouin zone. The $\beta'$ term with $\sigma_y$ appears because the edges of the Brillouin zone are more favorable for "diagonal" superpositions, such as $\Tilde{p}_x+\Tilde{p}_y$. 

% The key terms responsible for the formation of the WPs and for the topology of the bands arise from the circular-shaped Josephson currents which form due to the favorable phase differences at the interfaces \cite{suppl}. These terms, characterized by the constants $\alpha$ and $\xi$, enter the Hamiltonian with the $\sigma_z$ Pauli matrix, describing vortex states $\Tilde{p}_x+i\Tilde{p}_y$. In particular, the $\xi k_z\sigma_z$ term is responsible for the opening of the gap at the WPs when moving away from $\varphi_2=\pm\pi/2$.


% In the vicinity of a crossing point, the Hamiltonian~\eqref{Ham3D} can be reduced to the Weyl Hamiltonian:
% \begin{equation}
%     \hat{H}_{Weyl}=\bm{\eta} \bm{\sigma}\cdot \delta\bm{k},
%     \label{HWeyl}
% \end{equation}
% where $\bm{\sigma}=(\sigma_x,\sigma_y,\sigma_z)^T$, $\delta \bm{k}=(\delta k_x,\delta k_y,\delta k'_z)^T$ is the wavevector close to the WP and $\bm{\eta}=(2\sqrt{\Delta \beta},2\sqrt{\Delta\beta'^2/\beta},\xi)$. We define $\delta \bm{k}$ such as:
% \begin{equation}
%     \bm{k}=\left(\frac{\sqrt{\Delta}}{\sqrt{\beta}}\pm \delta k_x,\delta k_y, \frac{\alpha}{\xi} \delta k_y+\delta k_z\right)^T.
% \end{equation}
% This model is valid only in the vicinity of a WP and encodes most features associated with the energy spectrum, the pseudo-spin texture and the Berry curvature distribution.



%Alternatively, we define $\phi_2=-\phi_5+d_\phi$ which still gives 4 parameters but emphasizes the anti-symmetric behaviors of $\phi_{2,4}$ and $\phi_{4,5}$.
%The pentagonal geometry naturally breaks the inversion symmetry which is a necessary ingredient for the Weyl point existence. On the other hand the preservation of TR symmetry imposes that Weyl points are present by multiple of 4~\cite{nielsen1981absence,riwar2016multi}.% which form closed loops in the 4D parameter space (exactly as in~\cite{riwar2016multi}), and Weyl points in a 3D subspace. 



%These conditions together preserve TR symmetry~\cite{suppl}. 
%We focus on the two majority components of the $\Tilde{p}$ bands. Fig.~\ref{fig2}(a) shows for $\phi_2=\pi/2$ the bands plotted in the $\left (\phi_3,\phi_4 \right )$ subspace. The two 2D p-bands are well isolated from others (s and d). They are split everywhere, but degenerate in two linear crossing points along the diagonal direction $\phi_3=\phi_4$, which we now characterise further. Since we consider the two $\Tilde{p}$ bands, which are composed of states being linear combinations of $\Tilde{p}_x$ and $\Tilde{p}_y$, we can define the three following pseudo-spin components:

%The pseudospin texture allows to determine the effective field and to reconstruct the Weyl Hamiltonian at the crossing points, which are pseudo-spin singularities. %Having all 3 pseudospin components zero at the same time is impossible.



% Thus, the crossing point is a Weyl point in the synthetic space $\left (\phi_2,\phi_3,\phi_4 \right)$, which can be modeled by the Weyl Hamiltonian in its vicinity:
% \begin{equation}\label{WeylSynt}
%     \hat{H}_{Weyl}=\eta \bm{\sigma}\cdot \bm{\varphi},
% \end{equation}
% $\bm{\varphi}=\bm{\phi}-\bm{\phi}^{(0)}$ is the reduced parameter space in the vicinity of a Weyl point and $\bm{\sigma}$ is a vector containing the Pauli matrices $\sigma_{x,y,z}$. $\bm{\phi}=\left (\phi_2,\phi_3,\phi_4 \right)$ and $\bm{\phi}^{(0)}=\left (\phi_2^{(0)},\phi_3^{(0)},\phi_4^{(0)} \right)$ is a vector of the coordinates of the Weyl point in parameter space. The dispersion of a Weyl points varies linearly with a factor $\eta$ in each direction.



% ============================ Fig3 ============================ %
%\emph{Topological transition.--}
%We now  show that the Weyl points present in our system allow to probe different topological transitions between the two $\Tilde{p}$ bands simply by tuning the phase $\phi_2=-\phi_5$. We first consider the case $\phi_2=\pi/2$ where there are two Weyl points in the energy spectrum (see Fig.~\ref{fig2}(a)). The associated pseudo-spin is plotted in Fig.~\ref{fig3}(a), where the two Weyl points are easily identified as effective field singularities for the three components (source or sink for in-plane component and null circular component). However, there exist two other singularities of in-plane pseudo-spin located on the anti-diagonal. They correspond to gapped Weyl points because the $S_3$ component is non-zero. In this case, the Berry curvature (computed using the numerical method described in Ref.~\cite{fukui2005chern}, see~\cite{suppl})  shown in Fig.~\ref{fig3}(c) clearly shows the contribution of each of the 4 singularities: the two Weyl points do not contribute at all, whereas the gapped ones contribute with opposite signs. Then, decreasing slightly $\phi_2$ opens the gaps at the two Weyl points (as shown previously). The pseudo-spin is plotted in this case in Fig.~\ref{fig3}(b). The two $\Tilde{p}$ bands are now completely separated. The four in-plane pseudo-spin singularities are not concomitant with ill-definition of $S_3$ (which would translate into a green color), which proves that the bands are separated. This translates in the Berry curvature plotted in Fig.~\ref{fig3}(d). The anti-diagonal Weyl points still compensate each other, while the ones on the diagonal now contribute to the topology of the band with the same sign. Overall, the four singularities do not compensate. 
% We can write that at the Weyl points the effective field is zero and the pseudospin orientation is therefore arbitrary. 



%Further investigation shows that the two other Weyl points exist at $\phi_2\approx \pm \pi/4.5$ respectively, as depicted in Fig.~\ref{fig3}(f). These Weyl points are gapped for $\phi_2=\pi/2$ and correspond to the singularities in the in-plane pseudo-spin visible in Fig.~\ref{fig3}(a,b) on the anti-diagonal. These two Weyl points carry the same topological charge, opposite to the one of the two previously studied (see Fig.~\ref{fig3}(f) for clarity). The presence of these 4 Weyl points also allows reaching the transition from $\mathscr{C}_{gap}=\pm 1 $ to $\mathscr{C}_{gap}=0$, as shown in Fig.~\ref{fig3}(e). Starting from $\phi_2$ slightly higher than $\pi/2$, $\mathscr{C}_{gap}=+ 1 $, and keeping increasing $\phi_2$, the system encounters a unique Weyl point which  decreases the gap Chern number by 1: $\mathscr{C}_{gap}=0$. 

